IRKA is a Riemannian Gradient Descent Method

The iterative rational Krylov algorithm (IRKA) is a commonly used fixed-point iteration developed to minimize the $\mathcal{H}_2$ model order reduction error. In this work, IRKA is recast as a Riemannian gradient descent method with a fixed step size over the manifold of rational functions having fixed degree. This interpretation motivates the development of a Riemannian gradient descent method utilizing as a natural extension variable step size and line search. Comparisons made between IRKA and this extension on a few examples demonstrate significant benefits.

==> macros.tex <==
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsfonts}
\RequirePackage{mathtools}
\RequirePackage{dsfont}

% acronyms
\usepackage{acronym}
\acrodef{mor}[MOR]{model order reduction}

\acrodef{fom}[FOM]{full-order model}
\acrodef{rom}[ROM]{reduced-order model}

\acrodef{lti}[LTI]{linear time-invariant}
\acrodefindefinite{lti}{an}{a}

\acrodef{siso}[SISO]{single-input single-output}
\acrodef{mimo}[MIMO]{multiple-input multiple-output}

\acrodef{irka}[IRKA]{iterative rational Krylov algorithm}
\acrodef{irka2}[RGD-IRKA]{Riemannian Gradient Descent IRKA}

% MACROS
% \mathbb letters
\newcommand{\bbA}{\ensuremath{\mathbb{A}}}
\newcommand{\bbC}{\ensuremath{\mathbb{C}}}
\newcommand{\bbD}{\ensuremath{\mathbb{D}}}
\newcommand{\bbE}{\ensuremath{\mathbb{E}}}
\newcommand{\bbF}{\ensuremath{\mathbb{F}}}
\newcommand{\bbI}{\ensuremath{\mathbb{I}}}
\newcommand{\bbK}{\ensuremath{\mathbb{K}}}
\newcommand{\bbN}{\ensuremath{\mathbb{N}}}
\newcommand{\bbO}{\ensuremath{\mathbb{O}}}
\newcommand{\bbP}{\ensuremath{\mathbb{P}}}
\newcommand{\bbQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\bbR}{\ensuremath{\mathbb{R}}}
\newcommand{\bbS}{\ensuremath{\mathbb{S}}}
\newcommand{\bbU}{\ensuremath{\mathbb{U}}}
\newcommand{\bbV}{\ensuremath{\mathbb{V}}}
\newcommand{\bbX}{\ensuremath{\mathbb{X}}}
\newcommand{\bbY}{\ensuremath{\mathbb{Y}}}
\newcommand{\bbZ}{\ensuremath{\mathbb{Z}}}

% real vectors and matrices
\newcommand{\Rn}{\ensuremath{\bbR^{n}}}
\newcommand{\Rm}{\ensuremath{\bbR^{m}}}
\newcommand{\Rp}{\ensuremath{\bbR^{p}}}
\newcommand{\Rr}{\ensuremath{\bbR^{r}}}
\newcommand{\Rnn}{\ensuremath{\bbR^{n \times n}}}
\newcommand{\Rnm}{\ensuremath{\bbR^{n \times m}}}
\newcommand{\Rpn}{\ensuremath{\bbR^{p \times n}}}
\newcommand{\Rpm}{\ensuremath{\bbR^{p \times m}}}
\newcommand{\Rmn}{\ensuremath{\bbR^{m \times n}}}
\newcommand{\Rnr}{\ensuremath{\bbR^{n \times r}}}
\newcommand{\Rrr}{\ensuremath{\bbR^{r \times r}}}
\newcommand{\Rrm}{\ensuremath{\bbR^{r \times m}}}
\newcommand{\Rpr}{\ensuremath{\bbR^{p \times r}}}

% complex vectors and matrices
\newcommand{\Cn}{\ensuremath{\bbC^{n}}}
\newcommand{\Cm}{\ensuremath{\bbC^{m}}}
\newcommand{\Cp}{\ensuremath{\bbC^{p}}}
\newcommand{\Cr}{\ensuremath{\bbC^{r}}}
\newcommand{\Cnn}{\ensuremath{\bbC^{n \times n}}}
\newcommand{\Cnm}{\ensuremath{\bbC^{n \times m}}}
\newcommand{\Cpn}{\ensuremath{\bbC^{p \times n}}}
\newcommand{\Cpm}{\ensuremath{\bbC^{p \times m}}}
\newcommand{\Cmn}{\ensuremath{\bbC^{m \times n}}}
\newcommand{\Cnr}{\ensuremath{\bbC^{n \times r}}}
\newcommand{\Crr}{\ensuremath{\bbC^{r \times r}}}
\newcommand{\Crm}{\ensuremath{\bbC^{r \times m}}}
\newcommand{\Cpr}{\ensuremath{\bbC^{p \times r}}}

% \tilde letters
\newcommand{\tA}{\ensuremath{\tilde{A}}}
\newcommand{\tB}{\ensuremath{\tilde{B}}}
\newcommand{\tC}{\ensuremath{\tilde{C}}}
\newcommand{\tD}{\ensuremath{\tilde{D}}}
\newcommand{\tE}{\ensuremath{\tilde{E}}}
\newcommand{\tF}{\ensuremath{\tilde{F}}}
\newcommand{\tG}{\ensuremath{\tilde{G}}}
\newcommand{\tH}{\ensuremath{\tilde{H}}}
\newcommand{\tI}{\ensuremath{\tilde{I}}}
\newcommand{\tJ}{\ensuremath{\tilde{J}}}
\newcommand{\tK}{\ensuremath{\tilde{K}}}
\newcommand{\tL}{\ensuremath{\tilde{L}}}
\newcommand{\tM}{\ensuremath{\tilde{M}}}
\newcommand{\tN}{\ensuremath{\tilde{N}}}
\newcommand{\tO}{\ensuremath{\tilde{O}}}
\newcommand{\tP}{\ensuremath{\tilde{P}}}
\newcommand{\tQ}{\ensuremath{\tilde{Q}}}
\newcommand{\tR}{\ensuremath{\tilde{R}}}
\newcommand{\tS}{\ensuremath{\tilde{S}}}
\newcommand{\tT}{\ensuremath{\tilde{T}}}
\newcommand{\tU}{\ensuremath{\tilde{U}}}
\newcommand{\tV}{\ensuremath{\tilde{V}}}
\newcommand{\tW}{\ensuremath{\tilde{W}}}
\newcommand{\tX}{\ensuremath{\tilde{X}}}
\newcommand{\tY}{\ensuremath{\tilde{Y}}}
\newcommand{\tZ}{\ensuremath{\tilde{Z}}}
%
\newcommand{\ta}{\ensuremath{\tilde{a}}}
\newcommand{\tb}{\ensuremath{\tilde{b}}}
\newcommand{\tc}{\ensuremath{\tilde{c}}}
\newcommand{\td}{\ensuremath{\tilde{d}}}
\newcommand{\te}{\ensuremath{\tilde{e}}}
\newcommand{\tf}{\ensuremath{\tilde{f}}}
\newcommand{\tg}{\ensuremath{\tilde{g}}}
\newcommand{\tth}{\ensuremath{\tilde{h}}}
\newcommand{\ti}{\ensuremath{\tilde{\imath}}}
\newcommand{\tj}{\ensuremath{\tilde{\jmath}}}
\newcommand{\tk}{\ensuremath{\tilde{k}}}
\newcommand{\tl}{\ensuremath{\tilde{l}}}
\newcommand{\tm}{\ensuremath{\tilde{m}}}
\newcommand{\tn}{\ensuremath{\tilde{n}}}
\newcommand{\tto}{\ensuremath{\tilde{o}}}
\newcommand{\tp}{\ensuremath{\tilde{p}}}
\newcommand{\tq}{\ensuremath{\tilde{q}}}
\newcommand{\tr}{\ensuremath{\tilde{r}}}
\newcommand{\tss}{\ensuremath{\tilde{s}}}
\newcommand{\ttt}{\ensuremath{\tilde{t}}}
\newcommand{\tu}{\ensuremath{\tilde{u}}}
\newcommand{\tv}{\ensuremath{\tilde{v}}}
\newcommand{\tw}{\ensuremath{\tilde{w}}}
\newcommand{\tx}{\ensuremath{\tilde{x}}}
\newcommand{\ty}{\ensuremath{\tilde{y}}}
\newcommand{\tz}{\ensuremath{\tilde{z}}}
%
\newcommand{\tSigma}{\ensuremath{\tilde{\Sigma}}}
\newcommand{\tLambda}{\ensuremath{\tilde{\Lambda}}}

% calligraphic letters
\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cB}{\ensuremath{\mathcal{B}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}
\newcommand{\cF}{\ensuremath{\mathcal{F}}}
\newcommand{\cG}{\ensuremath{\mathcal{G}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\cJ}{\ensuremath{\mathcal{J}}}
\newcommand{\cK}{\ensuremath{\mathcal{K}}}
\newcommand{\cL}{\ensuremath{\mathcal{L}}}
\newcommand{\cM}{\ensuremath{\mathcal{M}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
\newcommand{\cO}{\ensuremath{\mathcal{O}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\cU}{\ensuremath{\mathcal{U}}}
\newcommand{\cV}{\ensuremath{\mathcal{V}}}
\newcommand{\cW}{\ensuremath{\mathcal{W}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}

% hat letters
\newcommand{\hA}{\ensuremath{\hat{A}}}
\newcommand{\hB}{\ensuremath{\hat{B}}}
\newcommand{\hC}{\ensuremath{\hat{C}}}
\newcommand{\hD}{\ensuremath{\hat{D}}}
\newcommand{\hE}{\ensuremath{\hat{E}}}
\newcommand{\hF}{\ensuremath{\hat{F}}}
\newcommand{\hG}{\ensuremath{\hat{G}}}
\newcommand{\hH}{\ensuremath{\hat{H}}}
\newcommand{\hI}{\ensuremath{\hat{I}}}
\newcommand{\hJ}{\ensuremath{\hat{J}}}
\newcommand{\hK}{\ensuremath{\hat{K}}}
\newcommand{\hL}{\ensuremath{\hat{L}}}
\newcommand{\hM}{\ensuremath{\hat{M}}}
\newcommand{\hN}{\ensuremath{\hat{N}}}
\newcommand{\hO}{\ensuremath{\hat{O}}}
\newcommand{\hP}{\ensuremath{\hat{P}}}
\newcommand{\hQ}{\ensuremath{\hat{Q}}}
\newcommand{\hR}{\ensuremath{\hat{R}}}
\newcommand{\hS}{\ensuremath{\hat{S}}}
\newcommand{\hT}{\ensuremath{\hat{T}}}
\newcommand{\hU}{\ensuremath{\hat{U}}}
\newcommand{\hV}{\ensuremath{\hat{V}}}
\newcommand{\hW}{\ensuremath{\hat{W}}}
\newcommand{\hX}{\ensuremath{\hat{X}}}
\newcommand{\hY}{\ensuremath{\hat{Y}}}
\newcommand{\hZ}{\ensuremath{\hat{Z}}}
%
\newcommand{\ha}{\ensuremath{\hat{a}}}
\newcommand{\hb}{\ensuremath{\hat{b}}}
\newcommand{\hc}{\ensuremath{\hat{c}}}
\newcommand{\hd}{\ensuremath{\hat{d}}}
\newcommand{\he}{\ensuremath{\hat{e}}}
\newcommand{\hf}{\ensuremath{\hat{f}}}
\newcommand{\hg}{\ensuremath{\hat{g}}}
\newcommand{\hh}{\ensuremath{\hat{h}}}
\newcommand{\hi}{\ensuremath{\hat{\imath}}}
\newcommand{\hj}{\ensuremath{\hat{\jmath}}}
\newcommand{\hk}{\ensuremath{\hat{k}}}
\newcommand{\hatl}{\ensuremath{\hat{l}}}
\newcommand{\hm}{\ensuremath{\hat{m}}}
\newcommand{\hn}{\ensuremath{\hat{n}}}
\newcommand{\ho}{\ensuremath{\hat{o}}}
\newcommand{\hp}{\ensuremath{\hat{p}}}
\newcommand{\hq}{\ensuremath{\hat{q}}}
\newcommand{\hr}{\ensuremath{\hat{r}}}
\newcommand{\hs}{\ensuremath{\hat{s}}}
\newcommand{\htt}{\ensuremath{\hat{t}}}
\newcommand{\hu}{\ensuremath{\hat{u}}}
\newcommand{\hv}{\ensuremath{\hat{v}}}
\newcommand{\hw}{\ensuremath{\hat{w}}}
\newcommand{\hx}{\ensuremath{\hat{x}}}
\newcommand{\hy}{\ensuremath{\hat{y}}}
\newcommand{\hz}{\ensuremath{\hat{z}}}
%
\newcommand{\hlambda}{\ensuremath{\hat{\lambda}}}
\newcommand{\hLambda}{\ensuremath{\hat{\Lambda}}}
\newcommand{\hdelta}{\ensuremath{\hat{\delta}}}
\newcommand{\hgamma}{\ensuremath{\hat{\gamma}}}

% calligraphic letters with hats
\newcommand{\hcA}{\ensuremath{\hat{\cA}}}
\newcommand{\hcB}{\ensuremath{\hat{\cB}}}
\newcommand{\hcC}{\ensuremath{\hat{\cC}}}
\newcommand{\hcD}{\ensuremath{\hat{\cD}}}
\newcommand{\hcE}{\ensuremath{\hat{\cE}}}
\newcommand{\hcF}{\ensuremath{\hat{\cF}}}
\newcommand{\hcG}{\ensuremath{\hat{\cG}}}
\newcommand{\hcH}{\ensuremath{\hat{\cH}}}
\newcommand{\hcI}{\ensuremath{\hat{\cI}}}
\newcommand{\hcJ}{\ensuremath{\hat{\cJ}}}
\newcommand{\hcK}{\ensuremath{\hat{\cK}}}
\newcommand{\hcL}{\ensuremath{\hat{\cL}}}
\newcommand{\hcM}{\ensuremath{\hat{\cM}}}
\newcommand{\hcN}{\ensuremath{\hat{\cN}}}
\newcommand{\hcO}{\ensuremath{\hat{\cO}}}
\newcommand{\hcP}{\ensuremath{\hat{\cP}}}
\newcommand{\hcQ}{\ensuremath{\hat{\cQ}}}
\newcommand{\hcR}{\ensuremath{\hat{\cR}}}
\newcommand{\hcS}{\ensuremath{\hat{\cS}}}
\newcommand{\hcT}{\ensuremath{\hat{\cT}}}
\newcommand{\hcU}{\ensuremath{\hat{\cU}}}
\newcommand{\hcV}{\ensuremath{\hat{\cV}}}
\newcommand{\hcW}{\ensuremath{\hat{\cW}}}
\newcommand{\hcX}{\ensuremath{\hat{\cX}}}
\newcommand{\hcY}{\ensuremath{\hat{\cY}}}
\newcommand{\hcZ}{\ensuremath{\hat{\cZ}}}

% function spaces
\newcommand{\Lone}{\ensuremath{\cL_{1}}}
\newcommand{\Ltwo}{\ensuremath{\cL_{2}}}
\newcommand{\Linf}{\ensuremath{\cL_{\infty}}}
\newcommand{\Lp}{\ensuremath{\cL_{p}}}
\newcommand{\Hone}{\ensuremath{\cH_{1}}}
\newcommand{\Htwo}{\ensuremath{\cH_{2}}}
\newcommand{\HtwoW}{\ensuremath{\cH_{2, W}}}
\newcommand{\Hinf}{\ensuremath{\cH_{\infty}}}
\newcommand{\Hp}{\ensuremath{\cH_{p}}}
\newcommand{\Hardy}{\ensuremath{\Htwo}}
\newcommand{\ReHardy}{\ensuremath{\Re\Hardy}}

% scaled parentheses, brackets, and braces
\DeclarePairedDelimiter{\myparen}{\lparen}{\rparen}
\DeclarePairedDelimiter{\mybrack}{\lbrack}{\rbrack}
\DeclarePairedDelimiter{\mybrace}{\lbrace}{\rbrace}

% real and imaginary parts
\newcommand{\imag}{\boldsymbol{\imath}}
\newcommand{\myconj}[1]{\ensuremath{\overline{#1}}}
\DeclarePairedDelimiterXPP{\Real}[1]{\operatorname{Re}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\Imag}[1]{\operatorname{Im}}{\lparen}{\rparen}{}{#1}

% matrix operators
\newcommand{\tran}{^{\operatorname{T}}}
\newcommand{\mtran}{^{-\!\operatorname{T}}}
\newcommand{\herm}{^{*}}
\newcommand{\mherm}{^{-*}}
\DeclarePairedDelimiterXPP{\eig}[1]{\sigma}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\sym}[1]{\operatorname{\mathsf{sym}}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\skw}[1]{\operatorname{\mathsf{skw}}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\vecop}[1]{\operatorname{\mathsf{vec}}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\mydiag}[1]{\operatorname{\mathsf{diag}}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\myspan}[1]{\operatorname{\mathsf{span}}}{\lbrace}{\rbrace}{}{#1}
\DeclarePairedDelimiterXPP{\orth}[1]{\operatorname{\mathsf{orth}}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\myrank}[1]{\operatorname{\mathsf{rank}}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\kernel}[1]{\operatorname{\mathsf{Ker}}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\image}[1]{\operatorname{\mathsf{Im}}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\trace}[1]{\operatorname{\mathsf{trace}}}{\lparen}{\rparen}{}{#1}

% functions
\newcommand{\fundef}[3]{\ensuremath{#1 \colon #2 \to #3}}
\DeclarePairedDelimiter{\card}{\lvert}{\rvert}
\DeclarePairedDelimiterXPP{\sign}[1]{\operatorname{sgn}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\rot}[1]{\operatorname{rot}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\curl}[1]{\operatorname{curl}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\divg}[1]{\operatorname{div}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\floor}[1]{}{\lfloor}{\rfloor}{}{#1}
\DeclarePairedDelimiterXPP{\ceil}[1]{}{\lceil}{\rceil}{}{#1}

% derivatives
\DeclareMathOperator{\dif}{d\!}
\newcommand{\D}{\ensuremath{\mathrm{D}}}
\newcommand{\diffd}{\ensuremath{\mathrm{d}}}

% floating-point numbers
\newcommand{\fln}[2]{\ensuremath{#1 \times 10^{- #2}}}
\newcommand{\flp}[2]{\ensuremath{#1 \times 10^{#2}}}

% norms
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiterXPP{\normF}[1]{}{\lVert}{\rVert}{_{\operatorname{F}}}{#1}
\DeclarePairedDelimiterXPP{\normone}[1]{}{\lVert}{\rVert}{_{1}}{#1}
\DeclarePairedDelimiterXPP{\normtwo}[1]{}{\lVert}{\rVert}{_{2}}{#1}
\DeclarePairedDelimiterXPP{\norminf}[1]{}{\lVert}{\rVert}{_{\infty}}{#1}
\DeclarePairedDelimiterXPP{\normLone}[1]{}{\lVert}{\rVert}{_{\Lone}}{#1}
\DeclarePairedDelimiterXPP{\normLtwo}[1]{}{\lVert}{\rVert}{_{\Ltwo}}{#1}
\DeclarePairedDelimiterXPP{\normLinf}[1]{}{\lVert}{\rVert}{_{\Linf}}{#1}
\DeclarePairedDelimiterXPP{\normLp}[1]{}{\lVert}{\rVert}{_{\Lp}}{#1}
\DeclarePairedDelimiterXPP{\normHone}[1]{}{\lVert}{\rVert}{_{\Hone}}{#1}
\DeclarePairedDelimiterXPP{\normHtwo}[1]{}{\lVert}{\rVert}{_{\Htwo}}{#1}
\DeclarePairedDelimiterXPP{\normHtwoW}[1]{}{\lVert}{\rVert}{_{\HtwoW}}{#1}
\DeclarePairedDelimiterXPP{\normHinf}[1]{}{\lVert}{\rVert}{_{\Hinf}}{#1}
\DeclarePairedDelimiterXPP{\normHp}[1]{}{\lVert}{\rVert}{_{\Hp}}{#1}

% inner product
\DeclarePairedDelimiterXPP{\ip}[2]{}{\langle}{\rangle}{}{#1, #2}
\DeclarePairedDelimiterXPP{\ipF}[2]{}{\langle}{\rangle}{_{\operatorname{F}}}{#1, #2}
\DeclarePairedDelimiterXPP{\ipLtwo}[2]{}{\langle}{\rangle}{_{\Ltwo}}{#1, #2}
\DeclarePairedDelimiterXPP{\ipHtwo}[2]{}{\langle}{\rangle}{_{\Htwo}}{#1, #2}
\DeclarePairedDelimiterXPP{\ipHtwoW}[2]{}{\langle}{\rangle}{_{\HtwoW}}{#1, #2}

% operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\subjectto}{subject\ to}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\Proj}{Proj}

% manifolds
\newcommand{\ManRat}{\ensuremath{\Sigma_{r, m, p}(\bbC)}}
\newcommand{\ReManRat}{\ensuremath{\Sigma_{r, m, p}(\bbR)}}
\newcommand{\ManRatStab}{\ensuremath{\Sigma_{r, m, p}^-(\bbC)}}
\newcommand{\ReManRatStab}{\ensuremath{\Sigma_{r, m, p}^-(\bbR)}}
\newcommand{\ManMat}{\ensuremath{S_{r, m, p}(\bbC)}}
\newcommand{\ReManMat}{\ensuremath{S_{r, m, p}(\bbR)}}
\newcommand{\ManMatStab}{\ensuremath{S_{r, m, p}^-(\bbC)}}
\newcommand{\ReManMatStab}{\ensuremath{S_{r, m, p}^-(\bbR)}}
\newcommand{\T}{\ensuremath{\mathrm{T}}}
\newcommand{\N}{\ensuremath{\mathrm{N}}}
\newcommand{\R}{\ensuremath{\mathrm{R}}}
\newcommand{\cauchy}{\ensuremath{\mathcal{CI}}}

% vectors
\newcommand{\ones}{\ensuremath{\mathds{1}}}

% overline
\newcommand{\of}{\ensuremath{\overline{f}}}
\newcommand{\onu}{\ensuremath{\overline{\nu}}}

% immersion
\newcommand{\immj}{\ensuremath{\mathbb{I}}}

% poles and residues
\newcommand{\lamik}{\lambda_{i}^{(k)}}
\newcommand{\bik}{b_{i}^{(k)}}
\newcommand{\cik}{c_{i}^{(k)}}
\newcommand{\lamikstar}{\overline{\lamik}}
\newcommand{\bikstar}{\myparen*{\bik}\herm}
\newcommand{\cikstar}{\myparen*{\cik}\herm}

